Optimization-Based Mechanical Perception for Peduncle Localization During Robotic Fruit Harvest

Rising global food demand and harsh working conditions make fruit harvest an important domain to automate. Peduncle localization is an important step for any automated fruit harvesting system, since fruit separation techniques are highly sensitive to peduncle location. Most work on peduncle localization has focused on computer vision, but peduncles can be difficult to visually access due to the cluttered nature of agricultural environments. Our work proposes an alternative method which relies on mechanical -- rather than visual -- perception to localize the peduncle. To estimate the location of this important plant feature, we fit wrench measurements from a wrist force/torque sensor to a physical model of the fruit-plant system, treating the fruit's attachment point as a parameter to be tuned. This method is performed inline as part of the fruit picking procedure. Using our orchard proxy for evaluation, we demonstrate that the technique is able to localize the peduncle within a median distance of 3.8 cm and median orientation error of 16.8 degrees.

==> sections/outline.tex <==

---INTRODUCTION---

\begin{itemize}
    \item For many crops, manual harvesting is still an unfortunate necessity.
    \begin{itemize}
        \item a lot of labor is needed for harvest \& food demand is increasing
        \item the work is physically demanding and a health risk
        \item no one wants to do it (labor stats)
        \item there has been strong research interest in robotic harvesting (cite harvesting papers or review(s))
    \end{itemize}
    \item Perception has been the main challenge in achieving this
    \begin{itemize}
        \item variation and occlusion make perception difficult in agricultural environments
        \item research has focused on vision-based fruit \& peduncle detection 
        \item viewpoint selection helps with occlusions but is limited by modality
        \item recent work on  mechanical perception holds promise but is limited by crop and requires isolated procedure
    \end{itemize}
    \item We propose a post-grasp (in-line?) exploratory procedure for online peduncle attachment point detection.
    \begin{itemize}
        \item we employ a physical modeling approach with optimization to  localize the attachment point
        \begin{itemize}
            \item This type of approach exists in the articulated object literature but is kinematic (ours is quasi-static & energy is exchanged)
        \end{itemize}
        \item procedure is executed between grasping and picking pattern, adding minimal time and ensuring adequate grasp
        \item Quick overview of techniques (model basis,  the physical proxy, basic testing procedure, etc.)
        \item Quick overview of results
    \end{itemize}
\end{itemize}

--- RELATED WORK ---

Possibly relevant subsections
\begin{itemize}
    \item selective harvesting for high-value crops (tomatoes, peppers, tree fruits)
    \item dealing with occlusions during perception tasks
    \item mechanical perception in and out of ag
\end{itemize}

Discuss the following:
Senden et al., "Exploiting plant dynamics in robotic fruit localization", 2022, -> model stem dynamics to estimate the location of tomato trusses

Lehnert et al., "Autonomous sweet pepper harvesting for protected cropping systems," 2017

An autonomous robot for harvesting cucumbers in greenhouses

Performance evaluation of a harvesting robot for sweet pepper

Development of a sweet pepper harvesting robot
